An Anytime Hierarchical Approach for Stochastic Task and Motion Planning

In order to solve complex, long-horizon tasks, intelligent robots need to carry out high-level, abstract planning and reasoning in conjunction with motion planning. However, abstract models are typically lossy and plans or policies computed using them can be inexecutable. These problems are exacerbated in stochastic situations where the robot needs to reason about and plan for multiple contingencies. We present a new approach for integrated task and motion planning in stochastic settings. In contrast to prior work in this direction, we show that our approach can effectively compute integrated task and motion policies whose branching structures encode agent behaviors that handle multiple execution-time contingencies. We prove that our algorithm is probabilistically complete and can compute feasible solution policies in an anytime fashion so that the probability of encountering an unresolved contingency decreases over time. Empirical results on a set of challenging problems show the utility and scope of our method.

==> conclusion.tex <==
\section{Conclusion}
In this paper, we formalize the \emph{stochastic task and motion planning (STAMP)} problem and introduce an \emph{anytime}, \emph{sound}, and \emph{probabilistically complete} \emph{HPlan} algorithm that uses \emph{entity} abstractions to compute contingent task and motion solutions for the STAMP problems using off-the-shelf task and motion planners. The \emph{HPlan} algorithm interleaves search for concretizations of the actions in the current model with computing refinements of the current abstract model. Policies generated through \emph{HPlan} are complete in the sense that it provides an action for each scenario that may arise while executing the policy, unlike previous works that provide partial policies for most likely scenarios only. The approach uses greedy selection to prioritize more likely actions over less likely ones to allow the robot to start executing actions rather than waiting for a complete solution. 

The approach assumes access to accurate descriptions for the robot's action models and an abstraction function that can be used to formulate the STAMP problem. As part of the future work, we intend to relax these assumptions by learning the abstraction function. \citet{shah2020learning} present a framework to learn critical regions for arbitrary motion planning problem. We plan to extend this work to learn the abstract representation for the STAMP problems. The current approach requires the robot to have full observability over its state. We also aim to relax this requirement and support partially observable setups as part of our future work. 



==> problem.tex <==
\section*{Problem Statement}

Let $\mathcal{O}$ be the set of symbolic references to the objects in the environment. For convenience, we will refer to these references directly as objects. 

Let $\mathcal{P}$ be a set of predicates. In this work, we consider two kinds predicates: \emph{symbolic} and \emph{hybrid}. We define each of them as follows: 
\begin{definition}
    Let $\mathcal{P}_{sym}$ be a set of \textbf{symbolic predicates} defined using a set of objects $o \subseteq \mathcal{O}$ as their arguments. 
\end{definition}

\begin{definition}
    Let $\mathcal{P}_{h}$ be a set of \textbf{concrete hybrid predicates}. Each $p_h(o,\Theta) \in \mathcal{P}_h$ uses a set of vectors $\Theta$ each of which is a vector of continuous values, along with the set of objects $o \subseteq \mathcal{O}$ as its arguments.
\end{definition}

A predicate $p \in \mathcal{P} = \mathcal{P}_{sym} \cup \mathcal{P}_h$ represents either a property of the object or a relation between two or more objects. For e.g., \emph{at($o_1$, loc)} specifies the location of the object $o_1$ where, $\{o_1\} \subset \mathcal{O}$ and \emph{loc} is a \emph{6-D} vector representing the pose of the object $o_1$ in the $3$-D environment, and \emph{on($o_x$, $o_y$)} specifies that object $o_x$ is placed on $o_y$.

Let $\alpha$ be a composition of entity abstraction (sec. \ref{sec:entity}) and function abstraction. For each concrete hybrid predicate $p_h \in \mathcal{P}_h$ we derive an abstract hybrid predicate $\abs{p_h}_{\alpha}$ as follows:  
\begin{definition}
    Let $ \llbracket \mathcal{P}_{h} \rrbracket_{\alpha}$ be a set of \textbf{abstract hybrid predicates}. Each $ \llbracket p_h \rrbracket_{\alpha} (o,\bar{\Theta}) \in \llbracket \mathcal{P}_{h} \rrbracket $ is an abstraction of its corresponding concrete predicate $p_h(o,\Theta) \in \mathcal{P}_h$, defined using a set of objects $o \subset \mathcal{O}$ and $\bar{\Theta}$ such that $\Theta \in \rho(\bar{\Theta})$.   
\end{definition}


We use predicates from $\mathcal{P}$ to define the concrete and abstract states as follows:

\begin{definition}
    A \textbf{concrete state} $x$ is defined as a subset of $\mathcal{P} = \mathcal{P}_{sym} \cup \mathcal{P}_h$. 
    $\mathcal{X}$ is a set of all possible concrete states. 
\end{definition}

\begin{definition}
    An \textbf{abstract state} $\abs{x}_{\alpha}$ is defined as a  subset of $ \llbracket \mathcal{P} \rrbracket_{\alpha} = \mathcal{P}_{sym} \cup \llbracket \mathcal{P}_h \rrbracket_{\alpha}$.  $\abs{\mathcal{X}}_{\alpha}$ is a set of all possible abstract states. 
\end{definition}

We classify actions available to the robot as \emph{symbolic} and \emph{hybrid} actions depending on the type predicates that appear in its actions. We define them as follows:

% \begin{definition}
%     Let $\llbracket \mathcal{X} \rrbracket_{\alpha}$ be the \textbf{abstract state space}. Each state $\llbracket x \rrbracket_{\alpha}$ is defined as a subset of $ \llbracket \mathcal{P} \rrbracket_{\alpha} = \mathcal{P}_{sym} \cup \llbracket \mathcal{P}_h \rrbracket_{\alpha}$.
% \end{definition}


\begin{definition}
    Let $\mathcal{A}_{sym}$ be a set of \textbf{symbolic actions} defined using predicates from $\mathcal{P}_{sym}$ such that $\forall a_{sym} \in \mathcal{A}_{sym},\, \emph{eff}_{a_{sym}} \subset \mathcal{P}_{sym}$.
\end{definition}


\begin{definition}
    Let $\mathcal{A}_h$ be a set of \textbf{concrete hybrid actions} defined using predicates from $\mathcal{P}_{sym} \cup \mathcal{P}_h$ such that $\forall a_{h} \in \mathcal{A}_{h},\, \emph{eff}_{a_{h}} \subset \mathcal{P}_{sym} \cup \mathcal{P}_h$.
\end{definition}
Each hybrid action $a_h \in \mathcal{A}_h$ is indeed 
% Each hybrid action $a_h \in \mathcal{A}_h$ is defined as 
a temporal abstraction of primitive actions that enable use of low-level controllers to manipulate the agent, and can be refined using a motion planner. For simplicity and without the loss of generality, we embed these refinements as parts of action arguments (see Fig. \ref{abs_example1}).


\begin{definition}
    Let $\llbracket \mathcal{A}_h \rrbracket_{\alpha}$ be a set of \textbf{abstract hybrid actions} defined using predicates from $\mathcal{P}_{sym} \cup \llbracket \mathcal{P}_{h} \rrbracket_{\alpha}$ such that $\forall \llbracket a_{h} \rrbracket_{\alpha} \in \llbracket \mathcal{A}_h \rrbracket_{\alpha},\, \emph{eff}_{\llbracket a_{h} \rrbracket_{\alpha}} \subset \mathcal{P}_{sym} \cup \llbracket \mathcal{P}_{h} \rrbracket_{\alpha}$.
\end{definition}

\begin{definition}
    A \textbf{concrete planning} problem $P$ is defined as a $6$-tuple $ P = \langle \mathcal{O}, \mathcal{P} = \mathcal{P}_{sym} \cup \mathcal{P}_h, \mathcal{X},  \mathcal{A} = \mathcal{A}_{sym} \cup \mathcal{A}_h, x_0, X_g \rangle$ where, $\mathcal{O}$ is a set of symbolic references to the objects in the environment, $\mathcal{P}$ is a set of predicates, $\mathcal{X}$ is a set of states, $\mathcal{A}$ is a set of actions available to the agent, $x_0 \in \mathcal{X}$ is an initial state, and $X_g \subset \mathcal{X}$ is a set of goal states.
    
\end{definition}

The solution to a concrete planning problem is a valid sequence of actions $\pi = \langle a_0,\dots,a_n \rangle$ such that $\forall a_i \in \pi,\, a_i \in  \mathcal{A}$ and when applied to $x_0$, the resultant state is $x_n \in X_g$.


\begin{definition}
    An \textbf{abstract planning} problem $\llbracket P \rrbracket_{\alpha}$ is defined as a $6$-tuple $ P = \langle \mathcal{O}, \llbracket \mathcal{P} \rrbracket_{\alpha} = \mathcal{P}_{sym} \cup \llbracket \mathcal{P}_h \rrbracket_{\alpha}, \llbracket \mathcal{X} \rrbracket_{\alpha},  \llbracket \mathcal{A} \rrbracket_{\alpha} = \mathcal{A}_{sym} \cup  \llbracket \mathcal{A}_h \rrbracket_{\alpha}, \llbracket x_0 \rrbracket_{\alpha}, \llbracket X_g \rrbracket_{\alpha} \rangle$ where, $\mathcal{O}$ is a set of symbolic references to the objects in the environment, $ \llbracket \mathcal{P} \rrbracket_{\alpha}$ is a set of abstract predicates, $\llbracket \mathcal{X} \rrbracket_{\alpha}$ is a set of abstract states, $\llbracket \mathcal{A} \rrbracket_{\alpha}$ is a set of abstract actions available to the agent, $\llbracket x_0 \rrbracket_{\alpha} \in \llbracket \mathcal{X} \rrbracket_{\alpha}$ is an initial state, and $\llbracket X_g \rrbracket_{\alpha} \subset \llbracket \mathcal{X} \rrbracket_{\alpha}$ is a set of goal states.
    
\end{definition}

The solution to an abstract planning problem is a valid sequence of actions $ \llbracket \pi \rrbracket_{\alpha} = \langle a_0,\dots,a_n \rangle$ such that  $\forall \llbracket a_i \rrbracket_{\alpha} \in \llbracket \pi \rrbracket_{\alpha},\, \llbracket a_i \rrbracket_{\alpha} \in  \llbracket \mathcal{A} \rrbracket_{\alpha}$ and when applied to $\llbracket x_0 \rrbracket_{\alpha}$, the resultant state is $\llbracket x_n \rrbracket_{\alpha} \in \llbracket X_g \rrbracket_{\alpha}$.

A \emph{concrete SSP} can be defined in a similar fashion with stochastic action descriptions for actions in $\mathcal{A}$.


% A \emph{concrete planning} problem $P$ is defined as a $5$-tuple $ P = \langle \mathcal{P}, \mathcal{X}, \mathcal{O}, \mathcal{A}, X_g \rangle$ where,  $\mathcal{P}$ is a set of predicates, $\mathcal{X}$ define a concrete state space that consists of states defined using the set of predicates $\mathcal{P}$, $\mathcal{O}$ defines a set of symbolic names for the objects in the environment, $\mathcal{A}$ is a set of actions available to the agent, and $X_g$ defines a set of goal states. Each state $x \in \mathcal{X}$ is made up of a subset of the set of predicates $ \mathcal{P}$. $\mathcal{P}$ is a union of sets $\mathcal{P}_{sym}$ and $\mathcal{P}_{h}$ where, $\mathcal{P}_{sym}$ is a set of symbolic predicates that use objects ffrom $\mathcal{O}$ as their arguments, and $\mathcal{P}_h$ is a set of hybrid predicates that use a set of real valued vectors $\theta$ along with symbolic arguments.  $\mathcal{A}$ defines a set of symbolic and hybrid actions defined using predicates from $\mathcal{P}$ and objects from $\mathcal{O}$. While every action $a \in \mathcal{A}$ affects the symbolic predicates in the state, hybrid actions also affects hybrid predicates. Hybrid actions are defined as a temporal abstraction of primitive actions that enable use of low-level controllers to manipulate the agent, and refined using a motion planner. For simplicity and without lose of generality, we embed these refinements as parts of action arguments (see Fig. \ref{abs_example1}). The solution to a concrete planning problem is a valid sequence of actions $[a_0,\dots,a_n]$ such that when applied to $x_0$, the resultant state is $x_n \in X_g$. 
% We use entity abstraction defined in the section \ref{sec:entity} to compute an abstract planning problem $[P]$ by abstracting the predicates with continuous vector $\theta$ using a set of symbolic arguments $[\theta]$. We then define set of abstract actions $[\mathcal{A}]$ with abstracted predicates. Fig. \ref{abs_example1} provides an example of one of the abstract actions where continuous parameters such as \emph{target\_pose} and robot configurations \emph{config$_1$} and \emph{config$_2$} are replaced by corresponding symbolic arguments. 

We define  task and motion planning problems as follows: 
\begin{definition}

    A \textbf{task and motion planning problem}  (\emph{TAMPP}) can be defined as a $5$-tuple $\langle \M$, $\alpha$, $\gamma$, $\abs{\M}_{\alpha} \rangle$ where, $\M$ is a concrete planning problem, $\alpha$ is an abstraction function that is composition of entity abstraction and function abstraction, $\gamma$ is a concretization function in the form of generators, and $\abs{\M}_{\alpha}$ is an abstract model computed by applying $\alpha$ on the concrete model $\M$.
\end{definition}

\begin{definition}

    A \textbf{stochastic task and motion planning problem}  (\emph{STAMPP}) can be defined as a $5$-tuple $\langle \M$, $\alpha$, $\gamma$, $\abs{\M}_{\alpha} \rangle$ where, $\M$ is a concrete \emph{SSP}, $\alpha$ is an abstraction function that is composition of entity abstraction and function abstraction, $\gamma$ is a concretization function in the form of generators, and $\abs{\M}_{\alpha}$ is an abstract model computed by applying $\alpha$ on the concrete model $\M$.
\end{definition}



Solutions to \emph{TAMPPs} or \emph{STAMPPs} are policies with actions from the concrete model $\M$. In this work, We consider solutions in the form of  a policy tree where each node $u_p$ in the tree represents an  state $s_{u_p}$ and edge $e_p$ represents an $a_{e_p}$. The child of a node-edge pair $(u_p,e_p)$ in the policy tree refers to a possible outcome of executing the action $a_{e_p}$ at the state $s_{u_p}$. In the case of all deterministic actions (\emph{TAMPP}), the tree would have a single branch. 

